Physics Briefing Book

The European Particle Physics Strategy Update (EPPSU) process takes a bottom-up approach, whereby the community is first invited to submit proposals (also called inputs) for projects that it would like to see realised in the near-term, mid-term and longer-term future. National inputs as well as inputs from National Laboratories are also an important element of the process. All these inputs are then reviewed by the Physics Preparatory Group (PPG), whose role is to organize a Symposium around the submitted ideas and to prepare a community discussion on the importance and merits of the various proposals. The results of these discussions are then concisely summarised in this Briefing Book, prepared by the Conveners, assisted by Scientific Secretaries, and with further contributions provided by the Contributors listed on the title page. This constitutes the basis for the considerations of the European Strategy Group (ESG), consisting of scientific delegates from CERN Member States, Associate Member States, directors of major European laboratories, representatives of various European organizations as well as invitees from outside the European Community. The ESG has the mission to formulate the European Strategy Update for the consideration and approval of the CERN Council.

==> BSM/authors.tex <==
\author{G.F. Giudice$^1$, P. Sphicas$^{1,2}$ {\rm (editors)},
J. Alcaraz$^3$, C. Doglioni$^4$
G. Lanfranchi$^{1,5}$, M. D'Onofrio$^6$, M. McCullough$^1$, 
G. Perez$^7$, P. Roloff$^1$, V. Sanz$^8$, A. Weiler$^9$, A. Wulzer$^{1,10,11}$
}

\institute{
$^1$ CERN, Geneva, Switzerland \\
$^2$ NKUA, Athens, Greece \\
$^3$ CIEMAT, Madrid, Spain \\
$^4$ Lund University, Lund, Sweden \\
$^5$ INFN-LNF, Frascati, Italy \\
$^6$ University of Liverpool, Liverpool, UK \\
$^7$ Weizmann Institute of Science, Tel Aviv, Israel \\
$^8$ University of Sussex, Sussex, UK \\
$^9$ Technical University of Munich, Munich, Germany \\
$^{10}$ EPFL, Lausanne, Switzerland \\
$^{11}$ University of Padova, Padova, Italy
}


==> Darkmatter/authors.tex <==
\author{Conveners: Marcela Carena$^1$, Shoji Asai$^2$ \\
Scientific secretaries: Christoph Weniger$^3$, Jocelyn Monroe$^4$, Caterina Doglioni$^5$,
Konstantinos Petridis$^6$, Gordan Krnjaic$^1$, Joerg Jaeckel$^7$, Babette D\"obrich$^8$ \\
%Speakers: Hitoshi Murayama$^{2,}$$^9$,
%Mariangela Lisanti$^{10}$,
%Matthew Philip Mccullough$^8$,
%Prateek Agrawal$^{11}$,
%Axel Lindner$^{12}$,
%Igor Garcia Irastorza$^{13}$,
%Claudia Frugiuele$^{8}$,\\
%Ruth Pottgen$^5$,
%Elena Graverini$^{8}$,
%Claude Vallee$^{14}$,
%Kathryn Zurek$^{15}$
}

\institute{
~\\
$^1$ Fermi National Accelerator Laboratory and the University of Chicago, USA \\
$^2$ The University of Tokyo, Japan \\
$^3$ GRAPPA, Institute of Physics, University of Amsterdam, Netherlands\\
$^4$ Royal Holloway, University of London, UK \\
$^5$ Lund, Sweden \\
$^6$ Bristol, UK \\
$^7$ Institut f\"ur theoretische Physik, Universit\"at Heidelberg, Germany \\
$^8$ CERN, Geneva, Switzerland \\
%$^9$ Berkeley, USA \\
%$^{10}$ Princeton University, USA \\
%$^{11}$ Harvard University, USA \\
%$^{12}$ DESY, Germany \\
%$^{13}$ Universidad de Zaragoza,  Spain \\
%$^{14}$ CPPM Marseille, France \\
%$^{15}$ Caltech, USA
}

==> Neutrino/sub1/mysubsec.tex <==
\subsection{Bibliography}
Keep each Section totally selfcontained, with
its own folder(s) for figures, and its own file for
bibliography~\cite{Mangano:2270978}.
Use bibtex format. Please get the bibtex from Inspire, other sources
may generate generate conflicts with the bibliography style file. For
internal notes of the LHC experiments, get the bibtex input from CDS
(the CERN Document Service). Each section must have its own bib
files. These are called \texttt{section.bib}, and should stay in the
folder
\verb|\main/mysection/bib/section.bib}|.
When you create a new section, add the bib file to the string
\begin{verbatim} 
\def\bibfiles{\main/bib/chapter,\main/section1/bib/section,\main/section2/bib/section}
\end{verbatim}
that is included in the main driver, report.tex.

In order for the references to be resolved you need to recompile \texttt{report.tex}. When you compile the other files it often does not work to resolved the references properly.







==> Neutrino/sub1/subsection.tex <==
\subsection{New subsection}
Here is a subsection



==> ewksection/bib/report.tex <==
https://www.overleaf.com/project/5ce2fbcc9743287397453459https://www.overleaf.com/project/5ce2fbcc9743287397453459

==> ewksection/extras.tex <==
\newpage
\subsection{Temporary repository for synergy suggestions}

\begin{itemize}
    \item EWK phase transition: LISA
    \item Fine structure constant measurements: AMO
\end{itemize}

\subsection{Temporary repository for cross references to be made with other sections}

\begin{itemize}
    \item need the accelerators to be defined in accelerator part by Lenny and Caterina.
    \item need the hierarchy problem to be discussed in introductory chapter by Gian
    \item reference to BSM section for DM and naturalness
    \item reference to flavor for CP
\end{itemize}

%\bibliography{\main/section1/bib/section}

\subsection{Things that could be put into an appendix or that are useful to keep while finalizing our chapter}
\begin{table}[]
    \centering
    \caption{Number of $Z$ bosons and $W$-pairs for each of the colliders at various $\sqrt{s}$ values. The LEP and SLC numbers reflect the numbers actually produced.
    \label{tab:ewkprogramme}
    \KE{LEP: 4 detectors, each with integrated luminosity of about 200 pb$^{-1}$
SLC: 600,000 measured, 350,000 in last two years.
LEP: numbers for W-pairs include production at threshold and above.}
\BH{CLIC 380, information by email from Philipp Rohloff assumes 50:50 split between +80\% and -80\% polarisation.}}
\begin{tabular}{l r|c c|cr|c|c}
         Collider                          & $\sqrt{s}$    & $\Delta t$ (yr) & $\int\cal{L}$d$t$ (\iab)& Particle & Number & Pol. & default plan \\\hline
         LEP\cite{ALEPH:2005ab}            & $\sim M_Z$    & 7 & $0.8\times 10^{-3}$ & Z-boson & $1.7\times 10^7$ & no & yes \\
         SLD\cite{ALEPH:2005ab}            & $\sim M_Z$    & 6 & ? & Z-boson & $6\times 10^5$ & yes & yes \\ 
         \FCCee\cite{Abada:2019zxq} & $\sim M_Z$ & 4 & $150$ & Z-boson & $3\times 10^{12}$ & no & yes \\
         \CEPC\cite{CEPCStudyGroup:2018ghi} & $\sim M_Z$    & 2  & $16$  & Z-boson &$3\times 10^{11}$ & no & yes\\ 
         \ILC\cite{ILCZ}                    & $\sim M_Z$    & 1-3  & $0.1$ & Z-boson & $4.9\times 10^9$ & yes & no \\
         \CLIC\cite{CLICZ}                  & $\sim M_Z$    & few  & $0.1$ & Z-boson & $5\times 10^9$ & yes & no \\ 
         \ILC\cite{ILCZ}                    & $250$ GeV     & 11  & $2$ & Z-boson & $1.1\times 10^8$ & yes & yes \\
         \CLIC\cite{CLICZ}                  & $380$~GeV     & 8 & $1$ & Z-boson & $5\times 10^6$ & yes & yes \\\hline
         LEP\cite{Schael:2013ita}          & $\gtrsim 2M_W$& 5 & $3\times 10^{-3}$ & W-pairs & $5\times 10^4$ & no & yes \\
         \FCCee\cite{Abada:2019zxq}    & $\sim 2M_W$   & 2 & $12$ & W-pairs & $1\times 10^6$ & no & yes \\
         \CEPC\cite{CEPCStudyGroup:2018ghi} & $\sim 2M_W$   & 1  & $2.6$ & W-pairs & $1.5\times 10^7$ & no &yes\\
         \CEPC\cite{CEPCStudyGroup:2018ghi} & $240$~GeV     & 7 & $5.6$ & W-pairs & $9.5\times 10^7$ & no & yes\\
         \FCCee\cite{Abada:2019zxq}    & $240$~GeV     & 4 & $5$ & W-pairs & $8.5\times 10^7$ & no & yes\\
         \ILC\cite{Fujii:2017vwa}           & $250$~GeV     & 11 & 2 & W-pairs & $3.4\times 10^7$ & yes & yes\\
         \CLIC                              & $380$~GeV     & 8 & 1 & W-pairs& $1.3\times 10^7$ & yes & yes\\
    \end{tabular}
\end{table}

\begin{table}[htbp]
    \centering
    \caption{Higgs coupling measurements from ATLAS~\cite{atlashcomb2}, using between $36.1$ and $79.8$~fb$^{-1}$ for most analyses, and CMS~\cite{cmshcomb2}, using $35.9$~fb$^{-1}$ for all analyses\label{tab:higgsnow}. For the ATLAS $\kappa_t$ result only the allowed values with $\kappa_t>0$ are shown. The \HLLHC projections are also shown based on Ref.~\cite{deBlas:2019rxi}. \BH{Removed table from main text as we now have a nice plot containing the information.}
    \label{higgsnow}
    }
    \begin{tabular}{c|r|r|r}
    \hline
    parameter & ATLAS & CMS & \HLLHC\\\hline\hline
       $\kappa_Z$, $\kappa_V\leq 1$ & $> 0.87$ at 95\% CL & $-0.87 \pm 0.09$& $> 0.987$ at 95\% CL\\
       $\kappa_W$, $\kappa_V\leq 1$ & $> 0.85$ at 95\% CL & $-1.00^{+0.09}_{-0.00}$& $> 0.983$ at 95\% CL\\
       $\kappa_b$  & $0.88 \pm 0.13$ & $0.91^{+0.17}_{-0.16}$ & $\pm 0.026$\\
       $\kappa_t$  & $[0.93,1.24]$ at 68\% CL & $1.02^{+0.19}_{-0.15}$ &$\pm 0.028$\\
       $\kappa_\tau$  & $0.97 \pm 0.13$ & $0.93\pm 0.13$ & $\pm 0.016$\\
       $\kappa_g$  & $1.01^{+0.13}_{-0.11}$ & $1.16^{+0.18}_{-0.13}$ & $\pm 0.022$\\
       $\kappa_\gamma$  & $0.98 \pm 0.07$ & $0.96 \pm 0.09$ & $\pm 0.017$\\
       $\kappa_\mu$  & n.a. & $0.72 ^{+0.50}_{-0.72}$ & $\pm 0.044$\\
$B(H\to \textrm{inv.})$ & $<0.30$ at 95\% CL & $<0.22$ at 95\% CL & $<0.019$ at 95\% CL\\
$B(H\to \textrm{undet.})$ & $<0.22$ at 95\% CL & $<0.38$ at 95\% CL & $<0.041$ at 95\% CL\\
\hline
    \end{tabular}
\end{table}


\begin{figure}[!ht]
\centering
\includegraphics[width=.8\linewidth]{\main/ewksection/img/Kappa0WithNewColumns}
\caption{\label{fig:hkappa0new}
Plot of kappa-0 with \FCChh only and \ILC1000 included.
}
\end{figure}



==> section1/sub1/mysubsec.tex <==
\subsection{Bibliography}
Keep each Section totally selfcontained, with
its own folder(s) for figures, and its own file for
bibliography~\cite{Mangano:2270978}.
Use bibtex format. Please get the bibtex from Inspire, other sources
may generate generate conflicts with the bibliography style file. For
internal notes of the LHC experiments, get the bibtex input from CDS
(the CERN Document Service). Each section must have its own bib
files. These are called \texttt{section.bib}, and should stay in the
folder
\verb|\main/mysection/bib/section.bib}|.
When you create a new section, add the bib file to the string
\begin{verbatim} 
\def\bibfiles{\main/bib/chapter,\main/section1/bib/section,\main/section2/bib/section}
\end{verbatim}
that is included in the main driver, report.tex.

In order for the references to be resolved you need to recompile \texttt{report.tex}. When you compile the other files it often does not work to resolved the references properly.







==> section1/sub1/subsection.tex <==
\subsection{New subsection}
Here is a subsection


